Systems-Theoretic Safety Assessment of Teleoperated Road Vehicles

Teleoperation is becoming an essential feature in automated vehicle concepts, as it will help the industry overcome challenges facing automated vehicles today. Teleoperation follows the idea to get humans back into the loop for certain rare situations the automated vehicle cannot resolve. Teleoperation therefore has the potential to expand the operational design domain and increase the availability of automated vehicles. This is especially relevant for concepts with no backup driver inside the vehicle. While teleoperation resolves certain issues an automated vehicle will face, it introduces new challenges in terms of safety requirements. While safety and regulatory approval is a major research topic in the area of automated vehicles, it is rarely discussed in the context of teleoperated road vehicles. The focus of this paper is to systematically analyze the potential hazards of teleoperation systems. An appropriate hazard analysis method (STPA) is chosen from literature and applied to the system at hand. The hazard analysis is an essential part in developing a safety concept (e.g., according to ISO26262) and thus far has not been discussed for teleoperated road vehicles.

==> Chapters/Archiv/Conclusion.tex <==
\section{\uppercase{Conclusions}}
\label{sec:conclusion}

\noindent 
{\color{red} short conclusion}



==> Chapters/Archiv/Methods.tex <==



==> Chapters/Archiv/Results.tex <==
\section{\uppercase{Results}}
\label{sec:results}
Vll genauer auf die Ergebnisse noch eingehen, Wie diese so aufgebaut sind.  Darauf eingehen was man an Konzeptuell berücksichtigen muss um ein Teleoperiertes System sicher zu gestalten.

Auch Zeigen dass man verschiedene Punkte durch Maßnahmen aus der Literatur schon umsetzen kann. Iteratives Vorgehen und Kontrollstruktur anpassen. ggf noch diskutieren dass dies ggf erst mal zu mehr UCAs und Scenarios führt ... Quantifizierung nötig (ASIL dazu ggf nicht geeignet, da es Fahrzeug nur ohne Sicherheitskonzept betrachtet -> Priorization FMEA)
\vfill
